Deep Anomaly Detection in Text

Deep anomaly detection methods have become increasingly popular in recent years, with methods like Stacked Autoencoders, Variational Autoencoders, and Generative Adversarial Networks greatly improving the state-of-the-art. Other methods rely on augmenting classical models (such as the One-Class Support Vector Machine), by learning an appropriate kernel function using Neural Networks. Recent developments in representation learning by self-supervision are proving to be very beneficial in the context of anomaly detection. Inspired by the advancements in anomaly detection using self-supervised learning in the field of computer vision, this thesis aims to develop a method for detecting anomalies by exploiting pretext tasks tailored for text corpora. This approach greatly improves the state-of-the-art on two datasets, 20Newsgroups, and AG News, for both semi-supervised and unsupervised anomaly detection, thus proving the potential for self-supervised anomaly detectors in the field of natural language processing.

==> chapters/results.tex <==
% !TEX TS-program = pdflatex


% ------------------------------------------------------------------------------
\chapter{Results}
\label{chp:results}
% ------------------------------------------------------------------------------

==> docs/arsclassica/Changes <==
2017/10/31
o Added compatibility with ClassicThesis 4.4

March 2017
o Fixed some details in the documentation

January 2017
o The subsection, subsubsection and paragraph titles are now in boldface
o Larger text body size
o Removed commands \arsincludegraphics, \ctLaTeX, \ctLaTeXe, \ctTeX: now the package has no commands at all 
o Fixed some details in the documentation and in arsclassica-settings file
o Rationalized "Changes" file

February 2012
o Fixed page numbers with "oneside" global option
o Caption package loaded
o Added compatibility with ClassicThesis 4.0
o Fixed some details in the documentation

June 2010
o Added compatibility with ClassicThesis 3.0 
o Removed language option: the package now has no option at all  
o In the documentation, bibliography made with biblatex package
o Documentation only in English 

February 2010
o Added compatibility with ClassicThesis 2.7

January 2009
o Corrected some typos in the documentation
o Documentation both in English and in Italian 
o Support for English, French, Spanish and German

December 2008
o The part numbers are now in Roman (uppercase) and not in roman (lowercase)
o Fixed some details in the documentation

November 2008
o First public release

==> docs/arsclassica/Chapters/Code.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%************************************************
\chapter{Code}
\label{chp:code}
%************************************************
 
\lstset{numbers=left,
    numberstyle=\scriptsize,
    stepnumber=1,
    numbersep=8pt
}    



Package announcement and request for necessary packages.
\begin{lstlisting}[firstnumber=1]
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{arsclassica}[2017/02/01]
\RequirePackage{classicthesis}
\RequirePackage{caption}
\end{lstlisting}



Text body size.
\begin{lstlisting}
\areaset[current]{370pt}{784pt}
\end{lstlisting}



Use of Iwona as font sans serif.
\begin{lstlisting}
\renewcommand{\sfdefault}{iwona}
\end{lstlisting}



Customized chapter numbers.
\begin{lstlisting}
\let\chapterNumber\undefined
\ifct@eulerchapternumbers
\newfont{\chapterNumber}{eurb10 scaled 5000}%
\else
\newfont{\chapterNumber}{pplr9d scaled 5000}%
\fi
\end{lstlisting}



Smallcaps sans serif.
\begin{lstlisting}
\ifthenelse{\boolean{@minionprospacing}}%
{%
  \DeclareRobustCommand{\spacedallcaps}[1]{\sffamily%
  \textssc{\MakeTextUppercase{#1}}}%
  \DeclareRobustCommand{\spacedlowsmallcaps}[1]%
  {\sffamily\textssc{\MakeTextLowercase{#1}}}%
}{%
  \ifthenelse{\boolean{@pdfspacing}}%
  {%
    \microtypesetup{expansion=false}%
    \DeclareRobustCommand{\spacedallcaps}[1]%
    {\sffamily\textls[160]{\MakeTextUppercase{#1}}}%
    \DeclareRobustCommand{\spacedlowsmallcaps}[1]%
    {\sffamily\textls[80]{\scshape\MakeTextLowercase{#1}}}%
  }{%
    \RequirePackage{soul} 
    \sodef\allcapsspacing{\sffamily\upshape}%
    {0.15em}{0.65em}{0.6em}%
    \sodef\lowsmallcapsspacing{\sffamily\scshape}%
    {0.075em}{0.5em}{0.6em}%   
    \DeclareRobustCommand{\spacedallcaps}[1]%
    {\MakeTextUppercase{\allcapsspacing{#1}}}%   
	\DeclareRobustCommand{\spacedlowsmallcaps}[1]%
	{\MakeTextLowercase{\textsc%
	   {\lowsmallcapsspacing{#1}}}}%
  }%
}
\end{lstlisting}



Semi-transparent headlines and page numbers in Iwona.
\begin{lstlisting}
\renewcommand{\sectionmark}[1]{\markright{\textsc%
{\MakeTextLowercase{\thesection}} \spacedlowsmallcaps{#1}}}
\lehead{\mbox{\llap{\small\thepage\kern1em\color{halfgray}\vline}%
\color{halfgray}\hspace{0.5em}\headmark\hfil}} 
\rohead{\mbox{\hfil{\color{halfgray}%
\headmark\hspace{0.5em}}%
\rlap{\small{\color{halfgray}\vline}\kern1em\thepage}}}
\renewcommand{\headfont}{\normalfont\sffamily}
\renewcommand{\pnumfont}{\small\sffamily}
\end{lstlisting}


  
Sectioning unit titles and description list labels in Iwona.
\begin{lstlisting}
\RequirePackage{titlesec}
    % parts
    \ifthenelse{\boolean{@parts}}%
    {%
    \titleformat{\part}[display]
        {\normalfont\centering\large}%
        {\thispagestyle{empty}\partname~\thepart}{1em}%
        {\color{Maroon}\spacedallcaps}
    }{\relax}
    % chapters
    \ifthenelse{\boolean{@linedheaders}}%
    {%
    \titleformat{\chapter}[display]%             
       {\relax}{\raggedleft{\color{halfgray}%
       \chapterNumber\thechapter} \\ }{0pt}%
       {\titlerule\vspace*{.9\baselineskip}\raggedright%
       \spacedallcaps}%
       [\normalsize\vspace*{.8\baselineskip}\titlerule]%
    }{%  
    \titleformat{\chapter}[block]%
       {\normalfont\Large\sffamily}%
       {{\color{halfgray}\chapterNumber\thechapter%
       \hspace{10pt}\vline}  }{10pt}%
       {\spacedallcaps}}
    % sections
    \titleformat{\section} 
       {\normalfont\Large\sffamily}{\textsc%
       {\MakeTextLowercase{\thesection}}}%
       {1em}{\spacedlowsmallcaps}
    % subsections
       \titleformat{\subsection}
       {\normalfont\sffamily\bfseries}{\textsc{\MakeTextLowercase%
       {\thesubsection}}}{1em}{\normalsize}
    % subsubsections
    \titleformat{\subsubsection}
       {\normalfont\sffamily\bfseries\itshape}{\textsc%
       {\MakeTextLowercase{\thesubsubsection}}}%
       {1em}{\normalsize\itshape}        
    % paragraphs
    \titleformat{\paragraph}[runin]
       {\normalfont\normalsize\sffamily\bfseries}{\textsc%
       {\MakeTextLowercase{\theparagraph}}}%
       {0pt}{\spacedlowsmallcaps}    
    % description labels
    \renewcommand{\descriptionlabel}[1]{\hspace*{\labelsep}%
    \bfseries\spacedlowsmallcaps{#1}}
    \titlespacing*{\chapter}{0pt}{1\baselineskip}{2\baselineskip}
    \titlespacing*{\section}{0pt}{2\baselineskip}%
       {.8\baselineskip}[\marginparsep]
    \titlespacing*{\subsection}{0pt}{1.5\baselineskip}%
       {.8\baselineskip}[\marginparsep]
    \titlespacing*{\paragraph}{0pt}{1\baselineskip}{1\baselineskip}

    \newcommand\formatchapter[1]{% 
    \vbox to \ht\strutbox{ 
    \setbox0=\hbox{\chapterNumber\thechapter\hspace{10pt}\vline\ } 
    \advance\hsize-\wd0 \advance\hsize-10pt\raggedright 
    \spacedallcaps{#1}\vss}} 
    \titleformat{\chapter}[block] 
       {\normalfont\Large\sffamily} 
       {\textcolor{halfgray}{\chapterNumber\thechapter} 
       \hspace{10pt}\vline\ }{10pt} 
    {\formatchapter}    

    \clearscrplain
    \rofoot[\mbox{\makebox[0pt][l]{\kern1em\thepage}}]{}
\end{lstlisting}



Itemize lists with semi-transparent labels.
\begin{lstlisting}
\renewcommand\labelitemi{\color{halfgray}$\bullet$} 
\end{lstlisting}



Caption settings.
\begin{lstlisting}
\captionsetup{format=hang,font=small,labelfont={sf,bf}}
\captionsetup[table]{skip=\medskipamount}
\end{lstlisting}



Hyper-reference settings.
\begin{lstlisting}
\hypersetup{
    colorlinks=true, linktocpage=true, pdfstartpage=1, 
    pdfstartview=FitV, breaklinks=true, pdfpagemode=UseNone, 
    pageanchor=true, pdfpagemode=UseOutlines,
    plainpages=false, bookmarksnumbered,
    bookmarksopen=true, bookmarksopenlevel=1,
    hypertexnames=true, pdfhighlight=/O,
    urlcolor=webbrown, linkcolor=RoyalBlue, 
    citecolor=webgreen,
    hyperfootnotes=false, pdfpagelabels,
    pdfcreator={pdfLaTeX},
    pdfproducer={LaTeX with ArsClassica}
}
\end{lstlisting}

==> docs/arsclassica/FrontBackMatter/Acknowledgements.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%*******************************************************
% Acknowledgements
%*******************************************************
\pdfbookmark{Acknowledgements}{Acknowledgements}

\chapter*{Acknowledgements}

\begin{flushright}
\itshape
We have seen that computer programming is an art, \\
because it applies accumulated knowledge to the world, \\
because it requires skill and ingenuity, \\
and especially because it produces objects of beauty. \\
\medskip
--- Donald Ervin Knuth
\end{flushright}

\bigskip
\bigskip

\heartpar{I wish first of all to thank the members of the Italian \TeX{} and \LaTeX{} User Group, in particular
Claudio Beccari, Fabiano Busdraghi, Gustavo Cevolani, Rosaria D'Addazio, Agostino De Marco, Massimiliano Dominici, Gloria Faccanoni, Claudio Fiandrino, Heinrich Fleck, Enrico Gregorio, Massimo Guiggiani, Roberto Giacomelli, Gianluca Gorni, Maurizio Himmelmann, Jer\'onimo Leal, Paride Legovini, Lapo Filippo Mori, Gianluca Pignalberi, Luigi Scarso, Marco Stara, Andrea Tonelli, Ivan Valbusa, Emiliano Giovanni Vavassori and Emanuele Vicentini,
for their invaluable aid during the writing of this work, the detailed explanations, the patience and the precision in the suggestions, the supplied solutions, the competence and the kindness: thank you, guys!
Thanks also to all the people who have discussed with me on the forum of the Group, prodigal of precious observations and good advices.
Finally, thanks to Andr\'e Miede, for his wonderful ClassicThesis style, and to Daniel Gottschlag, who gave to me the hint for this original reworking.}

==> docs/arsclassica/FrontBackMatter/Bibliography.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%*******************************************************
% Bibliography
%*******************************************************
\nocite{*}
\printbibliography

==> docs/arsclassica/FrontBackMatter/Contents.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%*******************************************************
% Contents
%*******************************************************
\phantomsection
\pdfbookmark{\contentsname}{tableofcontents}
\setcounter{tocdepth}{2}
\tableofcontents
\markboth{\spacedlowsmallcaps{\contentsname}}{\spacedlowsmallcaps{\contentsname}} 

==> docs/arsclassica/FrontBackMatter/Titleback.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%*******************************************************
% Titleback
%*******************************************************
\thispagestyle{empty}
\pdfbookmark{Titleback}{Titleback}

\hfill

\vspace{\stretch{2}}

\begin{center}
Lorenzo Pantieri \\
\smallskip
\textit{The \arsclassica{} package}\\
\smallskip
Copyright\,\textcopyright\ 2008-2017
\end{center}
\vspace{\stretch{1}}

\medskip

\noindent\textsf{\spacedlowsmallcaps{Titleback}} \\
\noindent
This document was written with \LaTeX{} on Mac using \arsclassica, a reworking of the \classicthesis{} style designed by Andr\'e Miede, inspired to the masterpiece \emph{The Elements of Typographic Style} by Robert Bringhurst. 

\bigskip

\noindent
\textsf{\spacedlowsmallcaps{Contacts}}

\noindent
{\raisebox{-0.33ex}{\ding{43}}}\,\mail{lorenzo.pantieri@gmail.com}

==> docs/arsclassica/FrontBackMatter/Titlepage.tex <==
% !TEX TS-program = pdflatex
% !TEX root = ../ArsClassica.tex

%*******************************************************
% Titlepage
%*******************************************************
\begin{titlepage}
\pdfbookmark{Titlepage}{Titlepage}
\changetext{}{}{}{((\paperwidth  - \textwidth) / 2) - \oddsidemargin - \hoffset - 1in}{}
    \begin{center}
        {\LARGE  

        \hfill

        \vfill

        {\spacedlowsmallcaps{\myName}} \\ \bigskip

        {\color{Maroon}\spacedallcaps{\myTitle}} 

        }

        \vfill

        \includegraphics[width=0.7\textwidth]{TFZSuperEllisse} \\ \bigskip

		\mySubTitle

        \vfill                      

    \end{center}        
\end{titlepage} 

==> docs/arsclassica/arsclassica-settings.tex <==
% ********************************************************************
% Personal commands
% ******************************************************************** 
\newcommand{\myName}{Lorenzo Pantieri}
\newcommand{\myTitle}{The ArsClassica package}
\newcommand{\mySubTitle}{Ah homage to the Elements of Typographic Style}

\DeclareRobustCommand*{\clsname}[1]{{\normalfont\sffamily#1}}
\DeclareRobustCommand*{\pkgname}[1]{{\normalfont\sffamily#1}}
\DeclareRobustCommand*{\optname}[1]{{\normalfont\ttfamily#1}}
\DeclareRobustCommand*{\cmdname}[1]{\mbox{\lstinline[basicstyle=\normalsize\ttfamily]!\\#1!}}

\DeclareRobustCommand*{\classicthesis}{Classic\-Thesis}
\DeclareRobustCommand*{\arsclassica}{{\normalfont\sffamily ArsClassica}}


% ********************************************************************
% Hyper-references
% ******************************************************************** 
\newcommand{\mail}[1]{\href{mailto:#1}{\texttt{#1}}}


% ********************************************************************
% Graphics
% ********************************************************************
\graphicspath{{Graphics/}}


% ********************************************************************
% Code
% ********************************************************************
\definecolor{lightergray}{gray}{0.99}

\lstset{language=[LaTeX]Tex,
     keywordstyle=\color{RoyalBlue},
     basicstyle=\small\ttfamily,
     commentstyle=\color{Emerald}\ttfamily,
     stringstyle=\rmfamily,
     numberstyle=\scriptsize,
     showstringspaces=false,
     breaklines=true,
     frame=lines,
     backgroundcolor=\color{lightergray},
     flexiblecolumns=true,
     escapeinside={£*}{*£},
     firstnumber=last,
} 

\newcommand{\meta}[1]{$\langle${\normalfont\itshape#1}$\rangle$}

\lstset{	morekeywords=%
    {ProvidesPackage,RequirePackage,areaset,ifthenelse,%
     chapterNumber,undefined,boolean,DeclareRobustCommand,%
     spacedallcaps,textssc,MakeTextUppercase,lehead,%
     microtypesetup,textls,spacedlowsmallcaps,MakeTextLowercase,%
     sodef,allcapsspacing,lowsmallcapsspacing,thesection,%
     color,headmark,rohead,headfont,pnumfont,titleformat,%
     part,partname,thepart,chapter,thechapter,titlerule,%
     subsection,thesubsection,subsubsection,thesubsubsection,%
     paragraph,theparagraph,descriptionlabel,titlespacing,%
     formatchapter,textcolor,clearscrplain,rofoot,labelitemi,
     captionsetup,hypersetup}}

\lstnewenvironment{code}% 
   {\setkeys{lst}{columns=fullflexible,keepspaces=true}%
   \lstset{basicstyle=\small\ttfamily}}{}


% ********************************************************************
% Bibliography
% ******************************************************************** 
\bibliography{Bibliography}

\defbibheading{bibliography}{%
\cleardoublepage
\manualmark
\phantomsection
\addcontentsline{toc}{chapter}{\tocEntry{\bibname}}
\chapter*{\bibname\markboth{\spacedlowsmallcaps{\bibname}}
{\spacedlowsmallcaps{\bibname}}}}

\renewcommand*{\nameyeardelim}{\addcomma\space}

==> docs/biblio.tex <==
% Manually add Bibliography to the TOC
\clearpage
\addcontentsline{toc}{chapter}{Bibliografie}

% Bibliography starts here
\begin{thebibliography}{99}
	\bibitem{curs}
		{Un Prof -- \emph{SuperCurs -- note de curs}}
	\bibitem{bk:a-book}
		{Autor1, Autor 2  --
			\emph{Book title} -- 1900 -- Editura}
	\bibitem{wk:xxx}
		{\emph{***, Software Developement Process} --\\
			\href{http://en.wikipedia.org/wiki/Software_development_process}
				{http://en.wikipedia.org/wiki/Software\_development\_process}
		}
\end{thebibliography}


==> docs/commands.tex <==
% Creates the text for referring to the figure identified by the key given as
% the first argument.
\newcommand{\figname}[1]{\emph{figura \ref{#1}}}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - label for the figure (used in \ref-ing the figure)
\newcommand{\insfig}[3]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				%\includegraphics[width=0.75\textwidth]{#1}
 				\includegraphics{#1}
			}
			\caption{#2\label{#3}}
			
	    \end{center}
	\end{figure}
}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - label for the figure (used in \ref-ing the figure)
%	#4 - fraction of the text width occupied by the figure
\newcommand{\insfigw}[4]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				\includegraphics[width=#4\textwidth]{#1}
			}
			\caption{#2\label{#3}}
			
	    \end{center}
	\end{figure}
}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - caption for display in the list of figures
%	#4 - label for the figure (used in \ref-ing the figure)
%	#5 - fraction of the text width occupied by the figure
\newcommand{\insfigshw}[5]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				\includegraphics[width=#5\textwidth]{#1}
			}
			\caption[#3]{#2\label{#4}}
			
	    \end{center}
	\end{figure}
}

==> docs/cover.tex <==
\thispagestyle{empty}
\begin{center}
\large
Universitatea „Politehnica” București \\
Facultatea de Automatică și Calculatoare \\
\vspace{\stretch{2}}

{\LARGE
	\textbf{Your overly impressing title here}
}

\vspace{3cm}
\textbf{Autor:}\\
Y'er name

\bigskip
\bigskip

\textbf{Coordonator științifici:}\\
prof. dr. ing. X Y\\

\vspace{\stretch{2}}
București\\
Iunie 2009 \\
\vspace*{1cm}
\end{center}


==> docs/highlight.tex <==
\usepackage{alltt}
\usepackage{marvosym}

\newcommand{\hlstd}[1]{\textcolor[rgb]{0,0,0}{#1}}
\newcommand{\hlnum}[1]{\textcolor[rgb]{0.53,0,0.13}{#1}}
\newcommand{\hlesc}[1]{\textcolor[rgb]{1,0,1}{\bf{#1}}}
\newcommand{\hlstr}[1]{\textcolor[rgb]{0.67,0.27,0}{#1}}
\newcommand{\hldstr}[1]{\textcolor[rgb]{0,0.53,0}{#1}}
\newcommand{\hlslc}[1]{\textcolor[rgb]{0.93,0.47,0}{#1}}
\newcommand{\hlcom}[1]{\textcolor[rgb]{1,0.53,0}{#1}}
\newcommand{\hldir}[1]{\textcolor[rgb]{0,0.53,0.27}{\bf{#1}}}
\newcommand{\hlsym}[1]{\textcolor[rgb]{0,0,0}{\bf{#1}}}
\newcommand{\hlline}[1]{\textcolor[rgb]{0.2,0.2,0.2}{#1}}
\newcommand{\hlkwa}[1]{\textcolor[rgb]{0.4,0.07,0.07}{\bf{#1}}}
\newcommand{\hlkwb}[1]{\textcolor[rgb]{0,0,0.4}{\bf{#1}}}
\newcommand{\hlkwc}[1]{\textcolor[rgb]{0,0,0.4}{#1}}
\newcommand{\hlkwd}[1]{\textcolor[rgb]{0,0.27,0.4}{#1}}
\definecolor{bgcolor}{rgb}{1,1,1}

==> docs/services-config.xml.tex <==
\noindent
\ttfamily
\hlstd{}\hlkwa{$<$?xml\ }\hlstd{}\hlkwb{version}\hlstd{=}\hlstr{"1.0"}\hlstd{\ }\hlkwb{encoding}\hlstd{=}\hlstr{"UTF{-}8"}\hlstd{}\hlkwa{?$>$}\hspace*{\fill}\\
\hlstd{}\hlkwa{$<$services{-}config$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ }\hlstd{}\hlkwa{$<$services$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$service{-}include\ }\hlstd{}\hlkwb{file{-}path}\hlstd{=}\hlstr{"remoting{-}config.xml"}\hlstd{\ }\hlkwa{/$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$default{-}channels$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ \ \ }\hlstd{}\hlkwa{$<$channel\ }\hlstd{}\hlkwb{ref}\hlstd{=}\hlstr{"my{-}amf"}\hlstd{}\hlkwa{/$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$/default{-}channels$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ }\hlstd{}\hlkwa{$<$/services$>$}\hspace*{\fill}\\
\hlstd{}\hlkwa{$<$/services{-}config$>$}\hlstd{}\hspace*{\fill}\\
\mbox{}
\normalfont


==> docs/template_diploma/biblio.tex <==
% Manually add Bibliography to the TOC
\clearpage
\addcontentsline{toc}{chapter}{Bibliografie}

% Bibliography starts here
\begin{thebibliography}{99}
	\bibitem{curs}
		{Un Prof -- \emph{SuperCurs -- note de curs}}
	\bibitem{bk:a-book}
		{Autor1, Autor 2  --
			\emph{Book title} -- 1900 -- Editura}
	\bibitem{wk:xxx}
		{\emph{***, Software Developement Process} --\\
			\href{http://en.wikipedia.org/wiki/Software_development_process}
				{http://en.wikipedia.org/wiki/Software\_development\_process}
		}
\end{thebibliography}


==> docs/template_diploma/commands.tex <==
% Creates the text for referring to the figure identified by the key given as
% the first argument.
\newcommand{\figname}[1]{\emph{figura \ref{#1}}}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - label for the figure (used in \ref-ing the figure)
\newcommand{\insfig}[3]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				%\includegraphics[width=0.75\textwidth]{#1}
 				\includegraphics{#1}
			}
			\caption{#2\label{#3}}
			
	    \end{center}
	\end{figure}
}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - label for the figure (used in \ref-ing the figure)
%	#4 - fraction of the text width occupied by the figure
\newcommand{\insfigw}[4]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				\includegraphics[width=#4\textwidth]{#1}
			}
			\caption{#2\label{#3}}
			
	    \end{center}
	\end{figure}
}

% Inserts a new figure, with these parameters:
%	#1 - filename of the figure to be inserted
%	#2 - caption for the figure
%	#3 - caption for display in the list of figures
%	#4 - label for the figure (used in \ref-ing the figure)
%	#5 - fraction of the text width occupied by the figure
\newcommand{\insfigshw}[5]{
	\begin{figure}[!htb]
		\begin{center}
			\fbox{
				\includegraphics[width=#5\textwidth]{#1}
			}
			\caption[#3]{#2\label{#4}}
			
	    \end{center}
	\end{figure}
}

==> docs/template_diploma/cover.tex <==
\thispagestyle{empty}
\begin{center}
\large
Universitatea „Politehnica” București \\
Facultatea de Automatică și Calculatoare \\
\vspace{\stretch{2}}

{\LARGE
	\textbf{Your overly impressing title here}
}

\vspace{3cm}
\textbf{Autor:}\\
Y'er name

\bigskip
\bigskip

\textbf{Coordonator științifici:}\\
prof. dr. ing. X Y\\

\vspace{\stretch{2}}
București\\
Iunie 2009 \\
\vspace*{1cm}
\end{center}


==> docs/template_diploma/highlight.tex <==
\usepackage{alltt}
\usepackage{marvosym}

\newcommand{\hlstd}[1]{\textcolor[rgb]{0,0,0}{#1}}
\newcommand{\hlnum}[1]{\textcolor[rgb]{0.53,0,0.13}{#1}}
\newcommand{\hlesc}[1]{\textcolor[rgb]{1,0,1}{\bf{#1}}}
\newcommand{\hlstr}[1]{\textcolor[rgb]{0.67,0.27,0}{#1}}
\newcommand{\hldstr}[1]{\textcolor[rgb]{0,0.53,0}{#1}}
\newcommand{\hlslc}[1]{\textcolor[rgb]{0.93,0.47,0}{#1}}
\newcommand{\hlcom}[1]{\textcolor[rgb]{1,0.53,0}{#1}}
\newcommand{\hldir}[1]{\textcolor[rgb]{0,0.53,0.27}{\bf{#1}}}
\newcommand{\hlsym}[1]{\textcolor[rgb]{0,0,0}{\bf{#1}}}
\newcommand{\hlline}[1]{\textcolor[rgb]{0.2,0.2,0.2}{#1}}
\newcommand{\hlkwa}[1]{\textcolor[rgb]{0.4,0.07,0.07}{\bf{#1}}}
\newcommand{\hlkwb}[1]{\textcolor[rgb]{0,0,0.4}{\bf{#1}}}
\newcommand{\hlkwc}[1]{\textcolor[rgb]{0,0,0.4}{#1}}
\newcommand{\hlkwd}[1]{\textcolor[rgb]{0,0.27,0.4}{#1}}
\definecolor{bgcolor}{rgb}{1,1,1}

==> docs/template_diploma/services-config.xml.tex <==
\noindent
\ttfamily
\hlstd{}\hlkwa{$<$?xml\ }\hlstd{}\hlkwb{version}\hlstd{=}\hlstr{"1.0"}\hlstd{\ }\hlkwb{encoding}\hlstd{=}\hlstr{"UTF{-}8"}\hlstd{}\hlkwa{?$>$}\hspace*{\fill}\\
\hlstd{}\hlkwa{$<$services{-}config$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ }\hlstd{}\hlkwa{$<$services$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$service{-}include\ }\hlstd{}\hlkwb{file{-}path}\hlstd{=}\hlstr{"remoting{-}config.xml"}\hlstd{\ }\hlkwa{/$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$default{-}channels$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ \ \ }\hlstd{}\hlkwa{$<$channel\ }\hlstd{}\hlkwb{ref}\hlstd{=}\hlstr{"my{-}amf"}\hlstd{}\hlkwa{/$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ \ \ }\hlstd{}\hlkwa{$<$/default{-}channels$>$}\hspace*{\fill}\\
\hlstd{}\hlstd{\ \ }\hlstd{}\hlkwa{$<$/services$>$}\hspace*{\fill}\\
\hlstd{}\hlkwa{$<$/services{-}config$>$}\hlstd{}\hspace*{\fill}\\
\mbox{}
\normalfont

